On the statistical evaluation of algorithmic's computational experimentation with infeasible solutions

The experimental evaluation of algorithms results in a large set of data which generally do not follow a normal distribution or are not heteroscedastic. Besides, some of its entries may be missing, due to the inability of an algorithm to find a feasible solution until a time limit is met. Those characteristics restrict the statistical evaluation of computational experiments. This work proposes a bi-objective lexicographical ranking scheme to evaluate datasets with such characteristics. The output ranking can be used as input to any desired statistical test. We used the proposed ranking scheme to assess the results obtained by the Iterative Rounding heuristic (IR). A Friedman's test and a subsequent post-hoc test carried out on the ranked data demonstrated that IR performed significantly better than the Feasibility Pump heuristic when solving 152 benchmark problems of Nonconvex Mixed-Integer Nonlinear Problems. However, is also showed that the RECIPE heuristic was significantly better than IR when solving the same benchmark problems.

==> mainText.old.tex <==
\section{Introduction} \label{sec:intro}

Algorithms are everywhere. They perform the most varied tasks, from solving theoretical problems, such as computing the minimum spanning tree of a given graph under some constraints~\cite{Zhang2012}, to practical problems, such as routing a vehicle between two cities while minimizing the fuel cost~\cite{Papadopoulos2018}. One can compare algorithms two ways: $(i)$ theoretically; and $(ii)$ empirically. The former analyzes their runtime and space complexities, while the latter usually rely on computational experiments performed on a predefined instances set.

The empirical evaluation of algorithms through computational experiment results in a large set of data that needs to be assessed by a statistical test. However, some entries of this dataset may be missing, which restricts the statistical evaluation. One cannot perform a variance test since its impossible to measure the average and the standard deviation of the dataset~\cite{Box2005}. In addition, data from computational experiments generally do not follow a normal distribution or are not heteroscedastic.~\cite{Garcia2009,Garcia2009b,Garcia2010}. Therefore, one should use a non-parametric statistical test instead of a parametric one~\cite{Weaver2017}.

The most common approach in the literature to deal with this problem is to ignore the missing data. Although being commonly used, this strategy erroneously neglects information regarding the algorithm's behavior. The work of Pavlikov~\cite{Pavlikov2018} is an example of such a wrong practice. In the result's discussion, the author excludes the data from instances where one of their algorithms cannot find feasible solutions in less than 50.000 seconds. Melo, Fampa, and Raupp~\cite{Melo2018} developed another work that has a similar approach. In their work, the instances with unfeasible solutions are ignored and the average result of each algorithm is reported. The work of Fortz, Oliveira, and Requejo~\cite{Fortz2017} also performs similarly and does not summarize the data from instances on which an algorithm cannot find feasible solutions within their time limit. It is worth noticing that none of these works run a statistical analysis on their data and only summarizes the average behavior of their algorithms.

Hence, the objective of this work is to formalize a non-parametric statistical analysis to evaluate datasets whose some of its entries may be missing. This paper proposes a statistical analysis based on the Friedman's test~\cite{Friedman1937}, which receives two data as input: $(i)$ the algorithms result; and $(ii)$ their running times. A case study is shown, using the proposed statistical analysis to evaluate the experiments of the Feasibility Pump heuristic~\cite{Fischetti2005}.

\section{The Friedman's test} \label{sec:friedman}

The Friedman rank sum test~\cite{Friedman1937} is a non-parametric randomized block analysis of variance test. Its null hypothesis states that no statistical difference was perceived among the evaluated treatments, while its alternative hypothesis states that a statistical difference was perceived. Since  Friedman's is a non-parametric test, it does not require the data to be from a normal distribution or %its residuals to have equal variance
to be heteroscedastic, \ie, its residuals have equal variance~\cite{Weaver2017}. Therefore, it is suitable to analyze data from algorithm experimentation when no data is missing. 

One can use the Friedman's test to detect differences among treatments (algorithms) across multiple trials (\eg, instances, inputs, datasets). This test receives as input a bi-dimensional vector $\textbf{A}_{m,n}$, where each column symbolizes a treatment and each row represents a trial. Furthermore, each cell $a_{i,j} \in \textbf{A}$ contains a real value that corresponds to the observation of test attempt $i$ by treatment $j$.

The test ranks each row of $\textbf{A}$ together, ranking the values by columns. The best treatment receives the rank $1$, the second best treatment receives the rank $2$, and so on. If there are tied values in a row, they receive the average of the ranks that would have been assigned without ties. Then, one can store the sum of each column into a vector $\textbf{S} = \{s_1, \ldots, s_n\}$, \ie, 
$$
  s_i = \sum_{j = 0}^m a_{i,j}.
$$ 
Using those values, the test statistics $FM$ is computed as in Equation~\eqref{eq:friedmanTestStatistics}, where $m$, $n$, and $s_i$ respectively denote the number of trials, the number of treatments, and the summation of the $i$-th column of $\textbf{A}$.

\begin{equation} \label{eq:friedmanTestStatistics}
    FM = \left ( \frac{12}{m  n  (n+1)} \sum_{i = 0}^n s_i^2 \right ) - 3  m  (n+1)
\end{equation}

Then, one must compare the $FM$ value with the \emph{critical difference value} $(CDF)$~\cite{Eisinga2017}. If $FM$ is greater or equal than $CDF$, then there is a significant difference between the analyzed treatments (and thus the null hypothesis is rejected) and a post-hoc test should be carried out. Otherwise, no significant difference is perceived and the null hypothesis is supported.

% fechei esta sessão

% One can verify if there is a statistical difference between two analyzed samples by checking if $FM$ is greater or equal to the \emph{critical difference value}.

% CONTINUAR AQUI

% http://www.statisticshowto.com/friedmans-test/
% http://www.portalaction.com.br/tecnicas-nao-parametricas/teste-de-friedman
% https://en.wikipedia.org/wiki/Friedman_test
% https://www.r-statistics.com/2010/02/post-hoc-analysis-for-friedmans-test-r-code/
% https://www.r-statistics.com/tag/friedman-test/

\section{A non-parametric statistical test for analyzing data of computational experiments with missing values} \label{sec:methodology}

This paper proposes a statistical analysis based on the Friedman's test to analyze data from computational experiments with missing values. It employs an additional initial step that builds the matrix $\textbf{A}$ by analyzing the algorithm's results and their running times. Then, the remaining of the test is unchanged.

It receives two bi-dimensional vectors as input: the first vector is denoted as $\textbf{R}_{m,n}$ and contains the algorithm's results, while the second vector is denoted as $\textbf{T}_{m,n}$ and 
contains the algorithm's running times. Let $\textbf{X}_{\textbf{k}} = \{x_1, \ldots, x_m\}$ be the $k$-th line of vector $\textbf{R}$ and 
$\textbf{Y}_{\textbf{k}} = \{y_1, \ldots, y_m\}$ 
be the $k$-th line of vector $\textbf{T}$. Assuming a minimization problem, one can build the $k$-th line of the matrix $\textbf{A}$ by ranking the input data according the following rules:

\begin{enumerate}
    \item If $x_i < x_j$, then $a_{ik} < a_{jk}$.
    \item If $x_i = x_j$, then $\left\{\begin{matrix}
a_{ik} < a_{jk}, & \text{if  } y_i < y_j.\\ 
a_{ik} > a_{jk}, & \text{if  } y_i > y_j.\\ 
a_{ik} = a_{jk}, & \text{if  } y_i = y_j.
\end{matrix}\right.$
    \item If $x_i$ is missing, then $\left\{\begin{matrix}
a_{ik} > a_{jk}, & \text{if  } a_{jk} \text{ is not missing}.\\ 
a_{ik} = a_{jk}, & \text{if  } a_{jk} \text{ is missing}.
\end{matrix}\right.$
\end{enumerate}

Rule $(1)$ states that, if algorithm $i$ achieves better results than algorithm $j$, then it ranked as superior. Rule $(2)$ is applied when two algorithms $i$ and $j$ achieve the same results. Then, the ranking decision is made by analyzing their running times. If algorithm $i$ runs in a smaller time than algorithm $j$, then algorithm $i$ is ranked as superior. On the other hand, if algorithm $i$ needs a greater computational time than algorithm $j$, then algorithm $j$ is ranked as superior. However, it both algorithm runs within the same time span, then they are ranked as equals. In this case, they receive the average of the ranks that would have been assigned without ties. Rule $(3)$ states that, if data from algorithm $i$ is missing (due to its inability to find feasible solutions in due time), then it is ranked equal as all other algorithms that also misses the data from the same trial. Besides, algorithm $i$ is ranked as inferior to any algorithm that finds feasible solutions in due time.

After building matrix $\textbf{A}$, the proposed statistical analysis proceeds as a classical Friedman's test, as described in Section~\ref{sec:friedman}.

\section{A case study} \label{sec:caseStudy}

This section presents a case study of the proposed statistical test by analyzing the data provided by Fischetti, Glover, and Lodi, on a work where they proposed the Feasibility Pump heuristic (FP)~\cite{Fischetti2005}. The FP is a constructive heuristic for general Mixed Integer Programming problems (MIP). One can use FP when MIP solvers cannot find feasible solutions without a significant computational effort. Since there are a lot of missing solution values on the aforementioned work (due to the incapacity of both the MIP solver and the FP to find feasible solutions), the proposed statistical test is especially suitable for analyzing its results.

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.8\textwidth}
        \includegraphics[width=\textwidth]{better.pdf}
        \caption{\label{subfig:better}}
    \end{subfigure}
    \begin{subfigure}{0.8\textwidth}
        \includegraphics[width=\textwidth]{worst.pdf}
        \caption{\label{subfig:worst}}
    \end{subfigure}
    \caption{Comparison of FP and CPLEX on instances where both algorithms find feasible solutions. Subfigure~ (\subref{subfig:better}) displays the instances where FP performs better than CPLEX, while Subfigure~(\subref{subfig:worst}) displays the instances where FP performs worst than CPLEX.}
    \label{fig:FPxCPLEX}
\end{figure*}

This case study evaluates the data provided in tables 3 and 4 of the above-mentioned paper. Those tables compare the FP with the CPLEX branch-and-bound for solving 83 difficult MIP problems from the literature, presenting, for each instance, the primal value and the running time of each algorithm. One can see that the FP cannot find feasible solutions for 3 instances, while the CPLEX branch-and-bound cannot achieve any feasible solution for 10 of the 83 evaluated instances. Since there are missing values, one cannot measure the treatments average and the standard deviation without dropping the missing data. Thus, a non-parametric rank-sum test is needed, from which the proposed statistical test is the most appropriated one.

Figure~\ref{fig:FPxCPLEX} summarizes the data of tables 3 and 4 of~\cite{Fischetti2005}. It shows, for 71 of the 83 evaluated instances, the quality of the FP solution in comparison to those of CPLEX. Subfigure~(\subref{subfig:better}) displays the instances on which FP obtained better solutions than CPLEX, while Subfigure~(\subref{subfig:worst}) displays the instances on which FP obtained worst solutions than CPLEX. The points on both graphs represent the ratio on which the better algorithm surpass the solution of the worst one, being computed as $\frac{FP}{CPLEX}$ and $\frac{CPLEX}{FP}$ on Subfigure~(\subref{subfig:better}) and Subfigure~(\subref{subfig:worst}), respectively. One can see that FP found better solutions than CPLEX on 39 instances. On the other hand, CPLEX achieved better solutions than FP on 29 instances. Both algorithms achieved the same results on 3 instances (\texttt{liu}, \texttt{ljb9}, and \texttt{lbj10}). In addition, FP found feasible solutions for 9 instances that CPLEX cannot achieve any integer solution (\texttt{momentum1}, \texttt{protfold}, \texttt{t1717}, \texttt{manpower1}, \texttt{manpower2}, \texttt{manpower3}, \texttt{manpower3a}, \texttt{manpower4}, and \texttt{manpower4a}). On the other hand, CPLEX found feasible solutions for 2 instances that FP cannot achieve any integer solution (\texttt{ds} and \texttt{p2756}). Both algorithms cannot achieve feasible solutions for a single instance (\texttt{rd-rplusc-21}). Therefore, FP found better solutions than CPLEX for 48 instances, whereas CPLEX outperforms FP on 32 instances.

The proposed test builds the matrix $\textbf{A}$ by applying the three rules presented in Section~\ref{sec:methodology} as follows. Using Rule (1), FP is ranked as superior to CPLEX on 39 of the 83 lines, while CPLEX is ranked as superior to FP on 29 lines. By applying Rule (2), FP is ranked as superior to CPLEX on 2 lines (FP achieved a smaller running time than CPLEX on instances \texttt{ljb9} and \texttt{lbj10}) and both algorithms are ranked as equals on a single line (they achieved the same running time on instance \texttt{liu}). Finally, Rule (3) ranks FP as superior to CPLEX on 9 lines and ranks CPLEX as superior to FP on 3 lines. Besides that, both algorithms are ranked as equals on 1 line (due to their inability to found feasible solutions for instance \texttt{rd-rplusc-21}).

Then, the proposed methodology applies a Friedman's test using the above-computed matrix $\textbf{A}$ as input. The Friedman's test was carried out on a Windows 64 bits PC using the R programming language version 3.5.1 and employed the \emph{friedman.test} function from the \emph{stats} package. The Friedman's test returned a $p$-value of $0.07364$. Then, the null hypothesis is supported, which means that no statistical difference was perceived between FP and CPLEX on the evaluated instances.

%\section{Conclusions}

%This paper proposed a statistical methodology to evaluate data from computational experiments where one or more algorithms cannot find feasible solutions for a subset of instances. The proposed methodology employs the Friedman's test with an additional preprocessing step. It is simple to use and can be easily implemented in any statistical software.
